Enabling Safety for Aerial Robots: Planning and Control Architectures

Ensuring safe autonomy is crucial for deploying aerial robots in real-world applications. However, safety is a multifaceted challenge that must be addressed from multiple perspectives, including navigation in dynamic environments, operation under resource constraints, and robustness against adversarial attacks and uncertainties. In this paper, we present the authors' recent work that tackles some of these challenges and highlights key aspects that must be considered to enhance the safety and performance of autonomous aerial systems. All presented approaches are validated through hardware experiments.

==> ICRA_2025_Ws/subsections/extra.tex <==
% @article{tordesillas2021faster,
%   title={Faster: Fast and safe trajectory planner for navigation in unknown environments},
%   author={Tordesillas, Jesus and Lopez, Brett T and Everett, Michael and How, Jonathan P},
%   journal={IEEE Transactions on Robotics},
%   volume={38},
%   number={2},
%   pages={922--938},
%   year={2021},
%   publisher={IEEE}
% }

% @article{singletary2022onboard,
%   title={Onboard safety guarantees for racing drones: High-speed geofencing with control barrier functions},
%   author={Singletary, Andrew and Swann, Aiden and Chen, Yuxiao and Ames, Aaron D},
%   journal={IEEE Robotics and Automation Letters},
%   volume={7},
%   number={2},
%   pages={2897--2904},
%   year={2022},
%   publisher={IEEE}
% }

% @ARTICLE{Dev_CDC_23_clarity,
%   author={Agrawal, Devansh R. and Panagou, Dimitra},
%   journal={IEEE Control Systems Letters}, 
%   title={Sensor-Based Planning and Control for Robotic Systems: Introducing Clarity and Perceivability}, 
%   year={2023},
%   volume={7},
%   number={},
%   pages={2623-2628},
%   keywords={Robot sensing systems;Entropy;Sea measurements;Trajectory;Estimation error;Kalman filters;Random variables;Information theory and control;Lyapunov methods;constrained control},
%   doi={10.1109/LCSYS.2023.3288493}}
